Multimodal Emotion Recognition in Conversations via Class-Wise Adaptive Modality Fusion and Affective Geometry

Emotion Recognition in Conversations (ERC) requires integrating heterogeneous textual, audio, and visual cues while accounting for conversational context and emotional dynamics. We extend the Self-Distillation Transformer architecture for ERC with appearance+geometry visual representations, class-wise adaptive modality fusion, and a valence-arousal prior for affective transitions. On the MELD and IEMOCAP datasets, geometry-enhanced visual representations improve weighted F1 by 0.27 and 4.36 points over appearance-only features, respectively, while class-wise adaptive fusion provides further gains of 0.17 and 0.25 points over the original softmax gate. The valence-arousal prior yields targeted improvements of 0.30 and 0.74 accuracy points on emotionally shifted utterances while preserving performance on stable turns. These results indicate that structured facial cues, emotion-dependent modality weighting, and affective geometry provide complementary benefits for multimodal ERC.

==> figures/valence_arousal_coords.tex <==
\newlength{\iemocapcolsep}
\newlength{\meldcolsep}
\setlength{\iemocapcolsep}{5.7pt}
\setlength{\meldcolsep}{4pt}

\begin{table}[t]
\centering
\caption{Valence-arousal coordinates for each emotion category in MELD
and IEMOCAP. MELD coordinates are fixed canonical positions derived from
Russell's circumplex~\cite{russell1980circumplex}.}
\label{tab:va_coords}
\renewcommand{\arraystretch}{1.3}

\resizebox{\columnwidth}{!}{%
\setlength{\tabcolsep}{\iemocapcolsep}
\begin{tabular}{lcccccc}
\hline
\multicolumn{7}{c}{\textbf{IEMOCAP}} \\
\hline
\textbf{Emotion} & Neutral & Happy & Excited & Angry & Sad & Frustrated \\
\hline
\textbf{Valence} & 0.50 & 0.80 & 0.75 & 0.20 & 0.20 & 0.25 \\
\textbf{Arousal} & 0.50 & 0.60 & 0.80 & 0.80 & 0.30 & 0.55 \\
\hline
\end{tabular}
}

\vspace{0.5em}

\resizebox{\columnwidth}{!}{%
\setlength{\tabcolsep}{\meldcolsep}
\begin{tabular}{lccccccc}
\hline
\multicolumn{8}{c}{\textbf{MELD}} \\
\hline
\textbf{Emotion} & Neutral & Joy & Surprise & Anger & Sadness & Fear & Disgust \\
\hline
\textbf{Valence} & 0.50 & 0.88 & 0.70 & 0.29 & 0.19 & 0.18 & 0.20 \\
\textbf{Arousal} & 0.50 & 0.74 & 0.84 & 0.84 & 0.37 & 0.80 & 0.68 \\
\hline
\end{tabular}%
}

\end{table}
